Hecke group algebras as quotients of affine Hecke algebras at level 0

The Hecke group algebra $HW_0$ of a finite Coxeter group $W_0$, as introduced by the first and last author, is obtained from $W_0$ by gluing appropriately its 0-Hecke algebra and its group algebra. In this paper, we give an equivalent alternative construction in the case when $W_0$ is the classical Weyl group associated to an affine Weyl group $W$. Namely, we prove that, for $q$ not a root of unity, $HW_0$ is the natural quotient of the affine Hecke algebra through its level 0 representation. We further show that the level 0 representation is a calibrated principal series representation for a suitable choice of character, so that the quotient factors (non trivially) through the principal central specialization. This explains in particular the similarities between the representation theory of the classical 0-Hecke algebra and that of the affine Hecke algebra at this specialization.

==> alcoves-B2.tex <==

\newlength\rootax
\newlength\rootay
\newlength\rootbx
\newlength\rootby
\newcommand{\setrootsystem}[2]{
  \gdef\theta{#1}
  \gdef\radius{#2}
  \pgfmathsetlength{\rootax}{\radius*cos(\theta/2)*cos(\theta/2)}
  \pgfmathsetlength{\rootay}{\radius*cos(\theta/2)*cos(180-\theta/2)}
  \pgfmathsetlength{\rootbx}{\radius*cos(\theta/2)*sin(\theta/2)}
  \pgfmathsetlength{\rootby}{\radius*cos(\theta/2)*sin(180-\theta/2)}
}
\newcommand{\drawHexagon}[2]{{
      \def\x{#1}
      \def\y{#2}
      \begin{scope}[xshift=  \x * 2*\rootax + \y * 2*\rootay,
                    yshift=  \x * 2*\rootbx + \y * 2*\rootby]
      \foreach \angle in { 0, \theta, ..., 360 }
      \draw[thick] (90+\angle-\theta/2:\radius) -- (90+\angle+\theta/2:\radius);
      \foreach \angle in { 0, \theta, ..., 360 }
      \draw[color=red,very thin]  (0,0) -- (90-\theta/2+2*\angle:\radius);
      \foreach \angle in { 0, \theta, ..., 180 }
      \draw[color=blue,very thin] (0,0) -- (90+\theta/2+2*\angle:\radius);
    \end{scope}
  }}

\setrootsystem{60}{2cm}
\begin{tikzpicture}[>=latex,join=bevel,scale=.5]
  \drawHexagon{-1}{-1}
  \drawHexagon{-1}{ 0}
  \drawHexagon{-1}{ 1}
  \drawHexagon{ 0}{-1}
  \drawHexagon{ 0}{ 0}
  \drawHexagon{ 0}{ 1}
  \drawHexagon{ 1}{-1}
  \drawHexagon{ 1}{ 0}
  \drawHexagon{ 1}{ 1}
\end{tikzpicture}




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 

